From Shadow Segmentation to Shadow Removal

The requirement for paired shadow and shadow-free images limits the size and diversity of shadow removal datasets and hinders the possibility of training large-scale, robust shadow removal algorithms. We propose a shadow removal method that can be trained using only shadow and non-shadow patches cropped from the shadow images themselves. Our method is trained via an adversarial framework, following a physical model of shadow formation. Our central contribution is a set of physics-based constraints that enables this adversarial training. Our method achieves competitive shadow removal results compared to state-of-the-art methods that are trained with fully paired shadow and shadow-free images. The advantages of our training regime are even more pronounced in shadow removal for videos. Our method can be fine-tuned on a testing video with only the shadow masks generated by a pre-trained shadow detector and outperforms state-of-the-art methods on this challenging test. We illustrate the advantages of our method on our proposed video shadow removal dataset.

==> snith.tex <==
begin{figure}[]
	\centering
  \includegraphics[width=0.9\textwidth]{figure/snith.png}
  \caption{\textbf{Image Shadow Removal using patch-based model.} In order to perform image shadow removal from patch shadow removal, we first extract shadow parameters and matte layers from each image patch lying on the shadow boundary. The shadow parameters of the whole image is the weighted sum of the shadow parameters of patches where the weight of the patch is its adversarial loss obtained from the discriminator D given the patch as input. We compute the image shadow matte similarly at each pixel location.}
  \label{fig:snith}

\end{figure}



Fig.\ref{fig:snith} visualizes this method. We show two shadow crops, their predicted shadow matte, their predicted shadow-free image patch, and the classification scores from D-Net. As can be seen, the classification score somewhat correlates to the quality of the generated patches. We use this score to weight the contribution of this patch parameters and matte layers to the image-level component. Note that we normalize all the classification scores to sum to 1. %To the best of our knowledge, we are the first to propose such a use of the critic function during inference for an image generation task.

